Designing a Virtual Reality Training Apprenticeship for Cold Spray Advanced Manufacturing

Apprenticeship and training programs in advanced manufacturing frequently encounter safety and accessibility concerns due to using heavy machinery. Virtual Reality (VR) training addresses such constraints while maintaining the spatial and procedural learning requirements of such training. However, designing effective VR training is challenging because advanced manufacturing processes are complex and require experts to train novices for a long time. This paper presents a VR Training Apprenticeship (VRTA) tailored for cold spray, which we carefully designed to teach novices step-by-step this particular advanced manufacturing process. To assess its effectiveness, we conducted an exploratory study ($n = 22$). We evaluated user experience (UX) measures in the form of quantitative scales, users' qualitative insights, and task performance with real-world machinery after the VR training. We discuss how the VRTA design contributed to the effectiveness and the challenges of considering VR training for advanced manufacturing.

==> TablesGraphs/corrsurvey.tex <==
\begin{table}[ht!]
\caption{Correlation matrix of survey and knowledge responses}
\label{tab:corrsurvey}
\begin{tabular}{|l|l|l|l|}
\hline
          & Pre VR    & Post VR   & Retention \\ \hline
Presence  & 0.162920  & -0.054728 & -0.193715 \\ \hline
Usability & -0.278425 & -0.265482 & -0.108352 \\ \hline
Nasa TLX  & -0.230299 & -0.410836 & -0.232344 \\ \hline
\end{tabular}
\end{table}

==> TablesGraphs/durations.tex <==
\begin{table}[hb!]
\centering
\caption{Player Time Spent in Minutes. }
\label{tab:durations}
\begin{tabular}{|cc|cc|cc|}
\hline
\multicolumn{2}{|c|}{Powder Feeder Time}       & \multicolumn{2}{c|}{Tutorial Time}   & \multicolumn{2}{c|}{Time per Step}  \\ \hline
\multicolumn{1}{|c|}{\textit{M}}       & \textit{SD }    & \multicolumn{1}{c|}{\textit{M}}      & \textit{SD}     & \multicolumn{1}{c|}{\textit{M}}     & \textit{SD }    \\ \hline
\multicolumn{1}{|c|}{26.9} & 12.6 & \multicolumn{1}{c|}{6.7} & 3.7 & \multicolumn{1}{c|}{1.1} & 2.4 \\ \hline
\end{tabular}
\end{table}

==> TablesGraphs/help.tex <==
\begin{table}[ht!]
\centering
\caption{VRTA assistance metrics.}
\label{tab:help}
\begin{tabular}{|cc|cc|cc|}
\hline
\multicolumn{2}{|c|}{Manual Hints} & \multicolumn{2}{c|}{Automatic Hints} & \multicolumn{2}{c|}{Step Reset}  \\ \hline
\multicolumn{1}{|c|}{\textit{M}}     & \textit{SD}   & \multicolumn{1}{c|}{\textit{M}}       & \textit{SD}    & \multicolumn{1}{c|}{\textit{M}}    & \textit{SD}   \\ \hline
\multicolumn{1}{|c|}{4.22}  & 6.12 & \multicolumn{1}{c|}{10.27}   & 2.94  & \multicolumn{1}{c|}{0.95} & 1.78 \\ \hline
\end{tabular}
\end{table}

==> TablesGraphs/knowledge.tex <==
\begin{table}[ht!]
\caption{Means and standard deviations of correct answers in knowledge questionnaires.}
\centering
\label{tab:Knowledge}
\begin{tabular}{|cc|cc|cc|}
\hline
\multicolumn{2}{|c|}{Pre VR}   & \multicolumn{2}{c|}{Post VR}     & \multicolumn{2}{c|}{Retention}   \\ \hline
\multicolumn{1}{|c|}{\textit{M}} & \textit{SD}   & \multicolumn{1}{c|}{\textit{M}}    & \textit{SD}   & \multicolumn{1}{c|}{\textit{M}}    & \textit{SD}   \\ \hline
\multicolumn{1}{|c|}{1} & 1.27 & \multicolumn{1}{c|}{4.18} & 2.08 & \multicolumn{1}{c|}{3.9} & 1.82 \\ \hline
\end{tabular}
\end{table}

==> TablesGraphs/qualtables.tex <==
%\subsubsection{Post VR}
%Our goal was to design and develop realistic VR training that emphasizes the learning goals, reduces the risk of motion sickness, and trains novices in a hands-on manner. Participants' responses are categorized based on the design decisions and the question's domain (questions are listed in the appendix). For the analysis, we used consensus validation and the results are in table ~\ref{PostVRTable}.

% maybe its better not to distinguish L and P? 
% I really think we should do the analysis base on questions cause they give context!

\begin{table*} [H]  \label{PostVRDomain}
    \centering
      \caption{Post-VR Survey; Based on Question Domains and Number of Occurrences}
    \footnotesize
    %\vspace{-0.5cm}
    \begin{tabular}{|p{3 cm}|p{2 cm}|p{1.5 cm}|p{2cm}|p{2 cm}|p{1.5 cm}|} \hline 
        \textbf{Design Sub-component} & \textbf{Preparedness} & \textbf{Realism} & \textbf{Helpful features} & \textbf{Unhelpful features} & \textbf{Training}\\ \hline 
        Tutorial & 0 &1 &3 &0 & 0 \\ \hline
          Environment Layout  & 0 &2 &0 & 1 & 0 \\ \hline
 Teleportation & 0 &2 &0 &1 & 0\\ \hline
  Visual/Audio Realism & 0 &6 &5 &0 & 0 \\ \hline
 VR Supervisor & 0 &0 &1 &0 & 0 \\ \hline
 Task Decomposition & 7 & 2 &8 & 5&0  \\ \hline
  Part info & 2 & 0& 0 & 0 &1 \\ \hline
   Why Statements& 1 &1 &0 &0 & 2 \\ \hline
  Auto Hints & 0 &1 &3 &0 & 0 \\ \hline
  Manual Hints & 0 &0 &1 &1 & 0 \\ \hline
  Animation & 0 &0 &0 &0 & 1  \\ \hline
 Auto Completion   & 0 &3 &0 &0 & 0  \\ \hline
  Confirmation  & 0 &1 &1 &0 & 1 \\ \hline
  Task Interactions   & 0 &3 &2 &6 & 0 \\ \hline
     
    \end{tabular}
   
    %\vspace{-0.5cm}
\end{table*}

\begin{table*} [H]  \label{PostVRPreparedness}
    \centering
      \caption{Post-VR Survey; Preparedness}
    \footnotesize
    %\vspace{-0.5cm}
    \begin{tabular}{|p{1.5 cm}|p{4.5 cm}|p{1 cm}|p{1 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|} \hline 
        \textbf{Design Sub-component} & \textbf{ Example Excerpt} & \textbf{Num. of Occurrence} &  \textbf{Positive Learning} & \textbf{Negative Learning}  &  \textbf{Positive Performance} & \textbf{Negative Performance} \\ \hline 
        Tutorial & - & - & - & - & - & - \\ \hline
          Environment Layout  & -& - & - & - &  & - \\ \hline
 Teleportation &- & - & - & - & - & -  \\ \hline
  Visual/Audio Realism & - & - & - & - & - & -  \\ \hline
 VR Supervisor &- & - & - & - & - & -  \\ \hline
  Task decomposition & P6: ''... the training provided clear steps and actions that reflect how I would dissemble and assemble the powder feeder in real life.''& 7 &  6 & 0 & 2& 0  \\ \hline
  Part info & P12:''...the VR helped show how to use the parts and what they are meant for.'' & 2 & 1 & 1 & 2 & 0  \\ \hline
   Why Statements & P9: ''I can more confidently work on the actual feeder now since I know the orientation of the parts and why they fit in a certain way which is necessary to prevent leaks and damages.'' & 1 & 1 & 0 & 1 & 0  \\ \hline
  Auto Hints& -& - & - & - & - & -  \\ \hline
  Manual Hints & - & - & - & - & - & -  \\ \hline
  Animation  &  -& - &- & - & - & -  \\ \
 Auto Completion   & - & - & - & - & - & -  \\ \hline
  Confirmation  & - & - & - & - & - & -  \\ \hline

  Task Interactions   & - & - & - & - & - & -  \\ \hline
     
    \end{tabular}
   
    %\vspace{-0.5cm}
\end{table*}



\begin{table*} [H]  \label{PostVRRealism}
    \centering
      \caption{Post-VR Survey; Realism}
    \footnotesize
    %\vspace{-0.5cm}
    \begin{tabular}{|p{1.5 cm}|p{4.5 cm}|p{1 cm}|p{1 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|} \hline 
        \textbf{Design Sub-component} & \textbf{ Example Excerpt} & \textbf{Num. of Occurrence} &  \textbf{Positive Learning} & \textbf{Negative Learning}  &  \textbf{Positive Performance} & \textbf{Negative Performance} \\ \hline 
        Tutorial & P14: ''...  I believe that a few more rounds of the tutorial and I would be able to perform the assembly/disassembly with minimal problems.'' & 1 & 0 & 0 & 1& 0 \\ \hline
          Environment Layout  & P23: ''The VR training was quite realistic in terms of the setup of the environment,'' & 2 & 2 & 0 & 2 & 0 \\ \hline
 Teleportation &  P16:'' …  easy to navigate'' & 2 & 0 & 0 & 0 & 0  \\ \hline
  Visual/Audio Realism & P17: ''… visuals and sound were simulated to be inside a factory.'' & 6 & 4 & 0 & 3 & 0  \\ \hline
 VR Supervisor &- & - & - & - & - & -  \\ \hline
  Task decomposition & P18: ''I find it somewhat realistic because it properly depicts all the parts and the steps... ''& 1 &  1 & 0 & 0& 0  \\ \hline
  Part info & - & - & - & - & - & -  \\ \hline
   Why Statements & P5: ''9/10. Great VR environment, actions such as unscrewing bolts felt smooth and logical...'' & 1 & 1 & 0 & 0 & 0  \\ \hline
  Auto Hints& -& - & - & - & - & -  \\ \hline
  Manual Hints & - & - & - & - & - & -  \\ \hline
  Animation  &  -& - &- & - & - & -  \\ \
 Auto Completion   & P6: ''I found it semi-realistic. This is because some of the steps were auto-completed after I initially put the tools or parts in their place which isn't realistic. However, the method was realistic.''& 3 & 0 & 0 & 1 & 2  \\ \hline
  Confirmation  & P14: ''I find it very realistic. It helps that after inserting a part or removing a part, it shows the correct way to perform the action.'' & 1 & 1 & 0 & 1 & 0  \\ \hline

  Task Interactions   &  P3: ''I would rate the realisticness of VR by 6/10. Because during the unscrewing of bolts, I wasn't able to unscrew them realistically.'' & 3 & 0 & 0 & 1 & 1  \\ \hline
     
    \end{tabular}
   
    %\vspace{-0.5cm}
\end{table*}



\begin{table*} [H]  \label{PostVRHelpful}
    \centering
      \caption{Post-VR Survey; Helpful Features}
    \footnotesize
    %\vspace{-0.5cm}
    \begin{tabular}{|p{1.5 cm}|p{4.5 cm}|p{1 cm}|p{1 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|} \hline 
        \textbf{Design Sub-component} & \textbf{ Example Excerpt} & \textbf{Num. of Occurrence} &  \textbf{Positive Learning} & \textbf{Negative Learning}  &  \textbf{Positive Performance} & \textbf{Negative Performance} \\ \hline 
        Tutorial & P23: ''The basic introduction on how to navigate the environment was really helpful. '' & 3 & 1 & 0 & 1& 0 \\ \hline
          Environment Layout  &- & - & - & - & - & - \\ \hline
 Teleportation & -& - & - & - & - & -  \\ \hline
  Visual/Audio Realism & P23:'' … An accurate scale of the working apparatus and the device gave the idea of what actually a powder feeder looks like ''& 5 & 3 & 0 & 2 & 0  \\ \hline
 VR Supervisor &P4: ''all of it especially the verbal guidance with the reason as to why that particular step is necessary'' & 1 & 1 & 0 & 0 & 0  \\ \hline
  Task decomposition & P11: ''Taking it step by step and having clear instructions..''& 8 &  8 & 0 & 4 & 0  \\ \hline
  Part info & - & - & - & - & - & -  \\ \hline
   Why Statements &- & - & - & - & - & -  \\ \hline
  Auto Hints& P12: ''Explaining the process and highlighting the parts which were to be used were very helpful.'' & 3 & 3 & 0 & 0 & 0  \\ \hline
  Manual Hints & P7: ''I would say the hints. Sometimes I couldn't understand what I need to do. At that time I clicked on hints and was able to complete the task'' & 1 & 0 & 0 & 1 & 0  \\ \hline
  Animation  &  -& - &- & - & - & -  \\ \
 Auto Completion   & - & - & - & - & - & -  \\ \hline
  Confirmation  &  P10: ''The videos showing how each action is done in real-time after you got the correct answer was a great way of checking yourself in my opinion '' & 1 & 0 & 0 & 1 & 0  \\ \hline

  Task Interactions   &  P14: ''Also added to the realism in that parts don't just click into place or screw pop in and out easily. I also believed the reasoning behind an action was valuable, helped in remembering dangers of doing a task wrong'' & 2 & 1 & 0 & 2 & 1  \\ \hline
     
    \end{tabular}
   
    %\vspace{-0.5cm}
\end{table*}



\begin{table*} [H]  \label{PostVRUnhelpful}
    \centering
      \caption{Post-VR Survey; Unhelpful Features}
    \footnotesize
    %\vspace{-0.5cm}
    \begin{tabular}{|p{1.5 cm}|p{4.5 cm}|p{1 cm}|p{1 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|} \hline 
        \textbf{Design Sub-component} & \textbf{ Example Excerpt} & \textbf{Num. of Occurrence} &  \textbf{Positive Learning} & \textbf{Negative Learning}  &  \textbf{Positive Performance} & \textbf{Negative Performance} \\ \hline 
        Tutorial & - & - & - & - & - & - \\ \hline
          Environment Layout  &P13: ''...Also for the gas line, the wrenches were not on the table like the rest of the tools, which threw me off.'' & 1 & 0 & 0 & 0 & 1 \\ \hline
 Teleportation & P19: ''Moving in the VR from one place to another was annoying''& 1 & 0 & 0 & 0 & 0  \\ \hline
  Visual/Audio Realism & -& - & - & - & - & -  \\ \hline
 VR Supervisor & - & - & - & - & - & -  \\ \hline
  Task decomposition &P14:'' I found it difficult to understand what some of the prompts wanted me to do, such as removing the rod underneath the lid - or more so - how to complete the task. When un/screwing the surrounding screws, I couldn't pick any screw which got me stuck a little bit.''& 5 &  0 & 5 & 0 & 2  \\ \hline
  Part info & - & - & - & - & - & -  \\ \hline
   Why Statements &- & - & - & - & - & -  \\ \hline
  Auto Hints&- & - & - & - & - & -  \\ \hline
  Manual Hints & P17:''How to place the spanner, bolts could have been highlighted, places where vacuum had to be put in'' & 1 & 0 & 1 & 0 & 0  \\ \hline
  Animation  &  -& - &- & - & - & -  \\ \
 Auto Completion   & - & - & - & - & - & -  \\ \hline
  Confirmation  & - & - & - & - & - & -  \\ \hline

  Task Interactions   & P8: ''lot of instructions and sometimes the screw tightening can be painful in handling with vr '' & 6 & 0 & 1 & 0 & 5  \\ \hline
     
    \end{tabular}
   
    %\vspace{-0.5cm}
\end{table*}

% I think we should remove this table, we asked the question for ourselves to get a better understanding of the future possibilities

\begin{table*} [H]  \label{PostVRTraining}
    \centering
      \caption{Post-VR Survey; Additional Training with VR}
    \footnotesize
    %\vspace{-0.5cm}
    \begin{tabular}{|p{1.5 cm}|p{4.5 cm}|p{1 cm}|p{1 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|} \hline 
        \textbf{Design Sub-component} & \textbf{ Example Excerpt} & \textbf{Num. of Occurrence} &  \textbf{Positive Learning} & \textbf{Negative Learning}  &  \textbf{Positive Performance} & \textbf{Negative Performance} \\ \hline 
        Tutorial & - & - & - & - & - & - \\ \hline
          Environment Layout  &- & - & - & - & - & - \\ \hline
 Teleportation & - & - & - & - & - & -   \\ \hline
  Visual/Audio Realism & -& - & - & - & - & -  \\ \hline
 VR Supervisor & - & - & - & - & - & -  \\ \hline
  Task decomposition & -& - & - & - & - & -  \\ \hline
  Part info & P12: ''When mentioning how to use certain parts like wavy spring I didn't know it was supposed to be rotated. Maybe a short demonstration of how it's to be performed would be helpful. '' & 1 & 0 & 1 & 0 & 0  \\ \hline
   Why Statements &P20: ''Spotting damages, and exercising more on the actual operations. Also, say, if one move goes wrong, what kind of damages will it lead to'' & 2 & 0 & 1 & 0 & 1  \\ \hline
  Auto Hints&- & - & - & - & - & -  \\ \hline
  Manual Hints &- & - & - & - & - & -  \\ \hline
  Animation  &  P6:'' I also liked that there was an arrow to show the orientation of the O-rings.''& 1 &1 & 0 & 0 & 0  \\ \
 Auto Completion   & - & - & - & - & - & -  \\ \hline
  Confirmation  & P21: ''...Doing the disassembly myself in 3D was confusing, but watching it being done in 3D was quite nice. What if we could watch it being disassembled in 3D first, and then do the step-by-step procedure? I think that would help viewers understand the process a bit better
'' & 1 & 1 & 0 & 1 & 0  \\ \hline

  Task Interactions   & P8: ''lot of instructions and sometimes the screw tightening can be painful in handling with vr '' & 6 & 0 & 1 & 0 & 5  \\ \hline
     
    \end{tabular}
   
    %\vspace{-0.5cm}
\end{table*}




%\subsubsection{Post Powder Feeder} 
%The participants filled out an open response questionnaire on the topic of preparedness and how the VR training affected their \textit{feeling} of preparedness concerning working on the \textit{Powder Feeder}. Questions are (1) How did the VR training help prepare you for the powder feeder task? (2) How did the VR training NOT help prepare you for the powder feeder task? (3) In what ways is the VR training different from actually working on the powder feeder? (4) What should be included in the VR training to make it more helpful? (5) Would you (still) use this VR training simulation to learn more about Cold Spray? Explain why. (6) After the powder feeder task, what training would you like to take to learn about the powder feeder?
%The VRTA's effectiveness is essentially tied to its ability to allow its users' ability to apply their training to real-life applications \cite{bossard_transfer_2008}, and their perceived confidence on the matter can effectively tell us about the training environment's usability \cite{may_mixed_2021}. 
%In table ~\ref{PostPFTable}, we highlighted the participants' feedback. 
%recheck the numbers here.

%\subsubsection{Post Powder Feeder} 
%The participants filled out an open response questionnaire on the topic of preparedness and how the VR training affected their \textit{feeling} of preparedness concerning working on the \textit{Powder Feeder}. Questions are (1) How did the VR training help prepare you for the powder feeder task? (2) How did the VR training NOT help prepare you for the powder feeder task? (3) In what ways is the VR training different from actually working on the powder feeder? (4) What should be included in the VR training to make it more helpful? (5) Would you (still) use this VR training simulation to learn more about Cold Spray? Explain why. (6) After the powder feeder task, what training would you like to take to learn about the powder feeder?
%The VRTA's effectiveness is essentially tied to its ability to allow its users' ability to apply their training to real-life applications \cite{bossard_transfer_2008}, and their perceived confidence on the matter can effectively tell us about the training environment's usability \cite{may_mixed_2021}. 
%In table ~\ref{PostPFTable}, we highlighted the participants' feedback. 
%recheck the numbers here.
\begin{table*} [H]  \label{PostPFTable}
    \centering
      \caption{Post-PF Participants' Feedback.}
    \footnotesize
    %\vspace{-0.5cm}
    \begin{tabular}{|p{1.5 cm}|p{4.5 cm}|p{1 cm}|p{1 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|} \hline 
        \textbf{Design Sub-component} & \textbf{ Example Excerpt} & \textbf{ Domain}& \textbf{ Num. of Occurrence} &  \textbf{Positive Learning} & \textbf{Negative Learning}  &  \textbf{Positive Performance} & \textbf{Negative Performance} \\ \hline 
        Tutorial & NA  & NA & NA & NA & NA & NA  \\ \hline
          Environment Layout  & P23: ''In VR all the steps were done easily in a standing upright position, whereas the actual feeder was more comfortable to do in a sitting position.'' & Realism & 5 & 1 & 1 & NA & 3 \\ \hline
 Teleportation & NA& NA & NA & NA & NA & NA  \\ \hline
  Visual/Audio Realism & P12: ''Not much different, the parts looked the same maybe the weight and power behind applying pressure was a little new'' & Realism & 10 & 3 & 1 & 4& 4  \\ \hline
 VR Supervisor & NA & NA & NA & NA & NA & NA  \\ \hline
  Task decomposition & P23:''It helped me a lot as I was familiarized with the steps on how to dissemble and re-assemble it, which I was clueless about how to do it first.'' & Preparedness& 11 & 7 & 2 & 2 & 1  \\ \hline
  Part info & P5:''Explanation of each piece, it's name, and it's function before it is introduced in context to the mechanism [is missing]'' & Suggestion features& 3 & 1 & 1& NA & NA  \\ \hline
   Why Statements &NA & NA & NA & NA & NA & NA  \\ \hline
  Auto Hints& NA & NA & NA & NA & NA & NA \\ \hline
  Manual Hints&NA & NA & NA & NA & NA & NA \\ \hline
  Animation  &NA & NA & NA & NA & NA & NA \\ \hline
 Auto Completion   &NA & NA & NA & NA & NA & NA \\ \hline
  Confirmation &NA & NA & NA & NA & NA & NA \\ \hline
  Task Interactions   & P11: '' some things actually felt easier in real life, especially working with the bolts and manipulating all the parts.'' & Realism & 3 & NA & NA & NA & 3  \\ \hline
     
    \end{tabular}
   
    %\vspace{-0.5cm}
\end{table*}

\begin{table*} [H]  \label{PostPFPreparedness}
    \centering
      \caption{Post-PF Survey; Preparedness}
    \footnotesize
    %\vspace{-0.5cm}
    \begin{tabular}{|p{1.5 cm}|p{4.5 cm}|p{1 cm}|p{1 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|} \hline 
        \textbf{Design Sub-component} & \textbf{ Example Excerpt} & \textbf{Num. of Occurrence} &  \textbf{Positive Learning} & \textbf{Negative Learning}  &  \textbf{Positive Performance} & \textbf{Negative Performance} \\ \hline 
        Tutorial & - & - & - & - & - & - \\ \hline
          Environment Layout  & P4:[not prepared ] ''...physically straining and the feel of using the tools in an actual setting, along with the orientation of the bolts (washer side up)'' & 1 & 0 & 1 & 0 & 0 \\ \hline
 Teleportation & - & - & - & - & - & -   \\ \hline
  Visual/Audio Realism & P12: ''Not much different, the parts looked the same maybe the weight and power behind applying pressure was a little new'' & 2 & 1 & 0 & 1 & 0  \\ \hline
 VR Supervisor & - & - & - & - & - & -  \\ \hline
  Task decomposition & P14: ''It did help a lot. The visual representation of the parts and the demonstration of how to perform the task helped retain a mental image of how the action must be done.'' & 6 & 5 & 0 & 2 & 0  \\ \hline
  Part info & P20: ''In the VR training, there is a small spring underneath the top lid, which was not mentioned in the VR training.'' & 1 & 0 & 1 & 0 & 0  \\ \hline
   Why Statements & - & - & - & - & - & -  \\ \hline
  Auto Hints & - & - & - & - & - & -  \\ \hline
  Manual Hints & - & - & - & - & - & -  \\ \hline
  Animation  &  - & - & - & - & - & -  \\ \
 Auto Completion   & - & - & - & - & - & -  \\ \hline
  Confirmation  & - & - & - & - & - & -  \\ \hline

  Task Interactions   & P19: ''The screwing and the physical things that need to be done (HAPTIC).'' & 1 & 0 & 0 & 0 & 1  \\ \hline
     
    \end{tabular}
   
    %\vspace{-0.5cm}
\end{table*}

\begin{table*} [H]  \label{PostPFRealism}
    \centering
      \caption{Post-PF Survey; Realism}
    \footnotesize
    %\vspace{-0.5cm}
    \begin{tabular}{|p{1.5 cm}|p{4.5 cm}|p{1 cm}|p{1 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|} \hline 
        \textbf{Design Sub-component} & \textbf{ Example Excerpt} & \textbf{Num. of Occurrence} &  \textbf{Positive Learning} & \textbf{Negative Learning}  &  \textbf{Positive Performance} & \textbf{Negative Performance} \\ \hline 
        Tutorial & - & - & - & - & - & - \\ \hline
          Environment Layout  &P12: ''Not much different, the parts looked the same maybe the weight and power behind applying pressure was a little new'' & 3 & 1 & 0 & 0 & 2 \\ \hline
 Teleportation & - & - & - & - & - & -   \\ \hline
  Visual/Audio Realism & -& - & - & - & - & -  \\ \hline
 VR Supervisor & - & - & - & - & - & -  \\ \hline
  Task decomposition & P17: ''VR gave few instruction and helped with each step, while in actual work no instruction to coordinate
'' & 1 & 0 & 0 & 0 & 1  \\ \hline
  Part info & - & - & - & - & - & -  \\ \hline
   Why Statements &P20: ''Spotting damages, and exercising more on the actual operations. Also, say, if one move goes wrong, what kind of damages will it lead to'' & 2 & 0 & 1 & 0 & 1  \\ \hline
  Auto Hints&- & - & - & - & - & -  \\ \hline
  Manual Hints &- & - & - & - & - & -  \\ \hline
  Animation  &  -  & - & - & - & - & - & -  \\ \hline
  Confirmation  & - & - & - & - & - & -  \\ \hline

  Task Interactions   & P21: ''The sizing of the Allen key used in the simulation was very different from the one in reality. I also found that it was phernominally easier to screw in the screws with my hands than with the wrenches, which seemed to be taking a long time. '' & 2 & 0 & 0 & 0 & 2  \\ \hline
     
    \end{tabular}
   
    %\vspace{-0.5cm}
\end{table*}

\begin{table*} [H]  \label{PostPFSuggestion}
    \centering
      \caption{Post-PF Survey; Suggested Features}
    \footnotesize
    %\vspace{-0.5cm}
    \begin{tabular}{|p{1.5 cm}|p{4.5 cm}|p{1 cm}|p{1 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|} \hline 
        \textbf{Design Sub-component} & \textbf{ Example Excerpt} & \textbf{Num. of Occurrence} &  \textbf{Positive Learning} & \textbf{Negative Learning}  &  \textbf{Positive Performance} & \textbf{Negative Performance} \\ \hline 
        Tutorial & - & - & - & - & - & - \\ \hline
          Environment Layout  & P14: ''...Also, one could add gravity to add overall more realism if you let go of things. And the VR could communicate noteworthy aspects of completing this task in real life that the operator should know. '' & 1 & 0 & 0 & 0 & 1 \\ \hline
 Teleportation & - & - & - & - & - & -   \\ \hline
  Visual/Audio Realism & P9: ''Graphics of the VR should be made better and there should be some way to differentiate weights while lifting heavy or lighter objects.'' & 4 & 0 & 1 & 2 & 2  \\ \hline
 VR Supervisor & - & - & - & - & - & -  \\ \hline
  Task decomposition & P1: ''The procedure should be divided into segments and the segments should be visible on the side. so i could know what happened will now and what is yet to come.''& 2 & 0 & 2 & 0 & 0  \\ \hline
  Part info & P111: ''... I think it would be cool if there were a part of the simulation where they can actually check that you remember the order correctly (maybe a task of like putting steps in order I'm not sure)'' & 1 & 1 & 0 & 0 & 0  \\ \hline
   Why Statements & - & - & - & - & - & -  \\ \hline
  Auto Hints & - & - & - & - & - & -  \\ \hline
  Manual Hints &- & - & - & - & - & -  \\ \hline
  Animation  & -  & - & - & - & - & - & -  \\ \hline
  Confirmation  & - & - & - & - & - & -  \\ \hline

  Task Interactions   & - & - & - & - & - & -  \\ \hline
     
    \end{tabular}
   
    %\vspace{-0.5cm}
\end{table*}


\begin{table*} [H]  \label{PostPFTraining}
    \centering
      \caption{Post-PF Survey; Suggested Features}
    \footnotesize
    %\vspace{-0.5cm}
    \begin{tabular}{|p{1.5 cm}|p{4.5 cm}|p{1 cm}|p{1 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|} \hline 
        \textbf{Design Sub-component} & \textbf{ Example Excerpt} & \textbf{Num. of Occurrence} &  \textbf{Positive Learning} & \textbf{Negative Learning}  &  \textbf{Positive Performance} & \textbf{Negative Performance} \\ \hline 
        Tutorial & - & - & - & - & - & - \\ \hline
          Environment Layout  & - & - & - & - & - & - \\ \hline
 Teleportation & - & - & - & - & - & -   \\ \hline
  Visual/Audio Realism & P21: ''I would, because it allows me to see all the parts in 3D without having to actually use the machine, which could likely be dangerous.'' & 1 & 1 & 0 & 0 & 0  \\ \hline
 VR Supervisor & - & - & - & - & - & -  \\ \hline
  Task decomposition & P17: ''yes sure since its intresting and stays helpful to remember the process once we start to focus on what the task is ''& 2 & 2 & 0 & 0 & 0  \\ \hline
  Part info & - & - & - & - & - & -  \\ \hline
   Why Statements & - & - & - & - & - & -  \\ \hline
  Auto Hints & - & - & - & - & - & -  \\ \hline
  Manual Hints &- & - & - & - & - & -  \\ \hline
  Animation  & -  & - & - & - & - & - & -  \\ \hline
  Confirmation  & - & - & - & - & - & -  \\ \hline

  Task Interactions   & - & - & - & - & - & -  \\ \hline
     
    \end{tabular}
   
    %\vspace{-0.5cm}
\end{table*}

%After two weeks, we asked participants about their experience and vivid memories of the tasks in VR. 


\begin{table*} [H]  \label{Retention}
    \centering
      \caption{Retention Survey}
    \footnotesize
    %\vspace{-0.5cm}
    \begin{tabular}{|p{1.5 cm}|p{4.5 cm}|p{1 cm}|p{1 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|} \hline 
        \textbf{Design Sub-component} & \textbf{ Example Excerpt} & \textbf{Num. of Occurrence} &  \textbf{Positive Learning} & \textbf{Negative Learning}  &  \textbf{Positive Performance} & \textbf{Negative Performance} \\ \hline 
        Tutorial & - & - & - & - & - & - \\ \hline
          Environment Layout  & P4:[not prepared ] ''...physically straining and the feel of using the tools in an actual setting, along with the orientation of the bolts (washer side up)'' & 1 & 0 & 1 & 0 & 0 \\ \hline
 Teleportation & - & - & - & - & - & -   \\ \hline
  Visual/Audio Realism & P12: ''Not much different, the parts looked the same maybe the weight and power behind applying pressure was a little new'' & 2 & 1 & 0 & 1 & 0  \\ \hline
 VR Supervisor & - & - & - & - & - & -  \\ \hline
  Task decomposition & P14: ''It did help a lot. The visual representation of the parts and the demonstration of how to perform the task helped retain a mental image of how the action must be done.'' & 6 & 5 & 0 & 2 & 0  \\ \hline
  Part info & P20: ''In the VR training, there is a small spring underneath the top lid, which was not mentioned in the VR training.'' & 1 & 0 & 1 & 0 & 0  \\ \hline
   Why Statements & - & - & - & - & - & -  \\ \hline
  Auto Hints & - & - & - & - & - & -  \\ \hline
  Manual Hints & - & - & - & - & - & -  \\ \hline
  Animation  &  - & - & - & - & - & -  \\ \
 Auto Completion   & - & - & - & - & - & -  \\ \hline
  Confirmation  & - & - & - & - & - & -  \\ \hline

  Task Interactions   & P19: ''The screwing and the physical things that need to be done (HAPTIC).'' & 1 & 0 & 0 & 0 & 1  \\ \hline
     
    \end{tabular}
   
    %\vspace{-0.5cm}
\end{table*}




%Moreover, participants highlighted important parts that affected their learning and helped in (dis)assembly of real PF. In table ~\ref{noneDD}, we highlighted these components. 

% update the numbers 
\begin{table*} [H]  \label{noneDD}
    \centering
      \caption{Participants' Feedback.}
    \footnotesize
    %\vspace{-0.5cm}
    \begin{tabular}{|p{1.5 cm}|p{4.5 cm}|p{1 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|} \hline 
        \textbf{Category} & \textbf{ Example Excerpt} & \textbf{ Num. of Occurrence} &  \textbf{Positive Learning} & \textbf{Negative Learning}  &  \textbf{Positive Performance} & \textbf{Negative Performance} \\ \hline 
       
  Making Mistakes & P4: ''... a virtual experience allowed me to make the mistakes I would have committed on the job and correct it helping me gain the extra know-how i needed to not mess up'' & - & 1 & NA & NA & -  \\ \hline
 Practical Experience & P8: ''I can now comforatably work on the powder feeder, it feels like you got a 
      Weight of Tools  & - & 1 & NA & NA & -  \\ \hline
       Safe Environment & P23: '' I think the actual cold spray environment might not be a safe place for a new person with no prior experience in it. It provides a safe environment where mistakes can be made without worrying about safety and damaging the equipment. '' & - & 1 & NA & NA & -  \\ \hline
    Cost-effective  & P4: '' yes, its cost-effective, I am allowed to mess up and learn from it '' & - & 1 & NA & NA & -  \\ \hline
       Crash Course & P5: '' It felt like a great crash course to learn about the cold spray process.'' & - & 1 & NA & NA & -  \\ \hline
           Interactivity & P14: ''I definitely would. It is interactive and I believe many people, including myself learn best in this hands-on manner.'' & - & 1 & NA & NA & -  \\ \hline
      Portable & P22: ''Yes, it is so convenient to use and I can learn the cold spray anywhere as long as I have the VR. '' & - & 1 & NA & NA & -  \\ \hline

    VR similar to real life& P7: ''Yeah, It helped me in many ways. It's exactly what I have seen and done in VR. I didn't find any difference or difficulty in how to disassemble or assemble this powder feeder.'' & - & 1 & NA & NA & -  \\ \hline
       Confident Builder & P11: '' I felt confident in the procedure because it felt like I had done it before. It felt very familiar and when I was remembering the training during  the process it felt more like remembering doing it for real.'' & - & 1 & NA & NA & -  \\ \hline
    Torques & P4: ''the tightening torque on the bolts were not known'' & - & 1 & NA & NA & -  \\ \hline
       Physical Feelings & P15: ''Probably with the feelings and physical touch parts required in the task. For example, when assembly back there is a need to rotate the drum to feel it locked in'' & - & 1 & NA & NA & -  \\ \hline
 Repeating & P1: ''Yes, I could redo the training or learn until i can work on the actual hardware'' & - & 1 & NA & NA & -  \\ \hline
      Fun & P9: ''Using VR to learn is more fun and engaging.'' & - & 1 & NA & NA & -  \\ \hline

    \end{tabular}
   
    %\vspace{-0.5cm}
\end{table&}


% what about retention?

==> TablesGraphs/reflectoniclite.tex <==
\begin{table}[]
\centering
\caption{Themes mentioned during the VRTG}
\label{tab:reflectonicslite}
\begin{tabular}{|cc|}
\hline
\multicolumn{2}{|c|}{\textbf{During VRTG}} \\ \hline
\multicolumn{1}{|c|}{Sequential}    & 35   \\ \hline
\multicolumn{1}{|c|}{Naming}     & 23   \\ \hline
\multicolumn{1}{|c|}{Others}        & 9    \\ \hline
\end{tabular}
\end{table}

==> TablesGraphs/surveytable.tex <==
\begin{table}[]
\caption{Mean and standard deviation of the Post VR survey responses}
\label{tab:survey}
\begin{tabular}{|cc|cc|cc|cc|cc|}
\hline
\multicolumn{2}{|c|}{Presence Scale} &
 \multicolumn{2}{c|}{Presence Overall} &
  \multicolumn{2}{c|}{Usability Scale} &
 \multicolumn{2}{c|}{Usability Overall} &
  \multicolumn{2}{c|}{NASA TLX} \\ \hline
\multicolumn{1}{|c|}{M} &
  SD &
 \multicolumn{1}{c|}{M} &
  SD &
  \multicolumn{1}{c|}{M} &
  SD &
\multicolumn{1}{c|}{M} &
  SD &
  \multicolumn{1}{c|}{M} &
  SD \\ \hline
\multicolumn{1}{|c|}{34.5} &
  4.87 &
  \multicolumn{1}{c|}{4.18} &
  0.66 &
  \multicolumn{1}{c|}{33.31} &
  5.69 &
  \multicolumn{1}{c|}{3.27} &
  0.88 &
  \multicolumn{1}{c|}{24.68} &
  5.2 \\ \hline
\end{tabular}
\end{table}

==> TablesGraphs/surveytable2.tex <==
\begin{table}[ht!]
\caption{Mean and standard deviation of the Post VR survey responses.}
%\setlength\tabcolsep{1 pt}
\centering
\label{tab:survey}
\begin{tabular}{|cc|cc|cc|cc|cc|}
\hline
\multicolumn{2}{|c|}{Presence} &
 % \multicolumn{2}{c|}{Presence Self} &
  \multicolumn{2}{c|}{Usability} &
  %\multicolumn{2}{c|}{Usability Self} &
  \multicolumn{2}{c|}{NASA TLX} \\ \hline
\multicolumn{1}{|c|}{\textit{M}} &
  \textit{SD} &
%  \multicolumn{1}{c|}{M} &
 % SD &
  \multicolumn{1}{c|}{\textit{M}} &
  \textit{SD} &
  %\multicolumn{1}{c|}{M} &
  %SD &
  \multicolumn{1}{c|}{\textit{M}} &
  \textit{SD} \\ \hline
\multicolumn{1}{|c|}{3.83} &
  0.54 &
%  \multicolumn{1}{c|}{4.18} &
 % 0.66 &
  \multicolumn{1}{c|}{3.7} &
  0.63 &
 % \multicolumn{1}{c|}{3.27} &
 % 0.88 &
  \multicolumn{1}{c|}{3.76} &
 0.95 \\ \hline
\end{tabular}
\end{table}

==> TablesGraphs/workloadTable.tex <==


\begin{table}[ht!]
\centering
\begin{tabular}{|cc|cc|cc|ll|ll|ll|ll|}
\hline
\multicolumn{2}{|c|}{Overall} &
  \multicolumn{2}{c|}{Mental} &
  \multicolumn{2}{c|}{Physical} &
  \multicolumn{2}{l|}{Temporal} &
  \multicolumn{2}{l|}{Effort} &
  \multicolumn{2}{l|}{Frustration} &
  \multicolumn{2}{l|}{Performance} \\ \hline
\multicolumn{1}{|c|}{M} &
  SD &
  \multicolumn{1}{c|}{M} &
  SD &
  \multicolumn{1}{c|}{M} &
  SD &
  \multicolumn{1}{l|}{M} &
  SD &
  \multicolumn{1}{l|}{M} &
  SD &
  \multicolumn{1}{l|}{M} &
  SD &
  \multicolumn{1}{l|}{M} &
  SD \\ \hline
\multicolumn{1}{|c|}{3.765} &
  0.948 &
  \multicolumn{1}{c|}{4.273} &
  1.453 &
  \multicolumn{1}{c|}{3.455} &
  1.595 &
  \multicolumn{1}{l|}{4.045} &
  1.397 &
  \multicolumn{1}{l|}{4.273} &
  1.279 &
  \multicolumn{1}{l|}{3.591} &
  1.869 &
  \multicolumn{1}{l|}{2.955} &
  0.899 \\ \hline
\end{tabular}
\caption{NASA-TLX Workload Breakdown}
\label{tab:Workload}
\end{table}

